Cuts in Graphs with Matroid Constraints

{\sc Vertex $(s, t)$-Cut} and {\sc Vertex Multiway Cut} are two fundamental graph separation problems in algorithmic graph theory. We study matroidal generalizations of these problems, where in addition to the usual input, we are given a representation $R \in \mathbb{F}^{r \times n}$ of a linear matroid $\mathcal{M} = (V(G), \mathcal{I})$ of rank $r$ in the input, and the goal is to determine whether there exists a vertex subset $S \subseteq V(G)$ that has the required cut properties, as well as is independent in the matroid $\mathcal{M}$. We refer to these problems as {\sc Independent Vertex $(s, t)$-cut}, and {\sc Independent Multiway Cut}, respectively. We show that these problems are fixed-parameter tractable ({\sf FPT}) when parameterized by the solution size (which can be assumed to be equal to the rank of the matroid $\mathcal{M}$). These results are obtained by exploiting the recent technique of flow augmentation [Kim et al.~STOC '22], combined with a dynamic programming algorithm on flow-paths \'a la [Feige and Mahdian,~STOC '06] that maintains a representative family of solutions w.r.t.~the given matroid [Marx, TCS '06; Fomin et al., JACM]. As a corollary, we also obtain {\sf FPT} algorithms for the independent version of {\sc Odd Cycle Transversal}. Further, our results can be generalized to other variants of the problems, e.g., weighted versions, or edge-deletion versions.

==> matroidprelims.tex <==

\paragraph{Matroids.}  We refer to the textbook of Oxley~\cite{Oxley11} for the introduction to Matroid Theory. Here we only briefly introduce the most important notions.
\begin{definition}[Matroid]\label{def:matroid}
	A pair $\cM=(V,\cI)$, where $V$ is a \emph{ground set} and $\cI$ is a family of subsets, called \emph{independent sets of $\cM$}, is a \emph{matroid} if it satisfies the following conditions, called \emph{independence axioms}:
	\begin{itemize}
		\item  $\emptyset\in \cI$, 
		\item if $X \subseteq Y $ and $Y\in \cI$ then $X\in\cI$, 
		\item if $X,Y  \in \cI$  and $ |X| < |Y| $, then there is $v\in  Y \setminus X $  such that $X\cup\{v\} \in \cI$.
	\end{itemize}
\end{definition}
We use $V(\cM)$ and $\cI(\cM)$ to denote the ground set and the family of independent sets of $\cM$, respectively, unless $\cM$ is clear from the context.   
An inclusion-maximal set of $\cI$ is called a \emph{base}; it is well-known that all bases of $\cM$ have the same cardinality.
A function $r\colon 2^V\rightarrow \mathbb{Z}_{\geq 0}$  such that for every $X\subseteq V$,
\begin{center}
	
	$ 	r(X)=\max\{|Y|\colon Y\subseteq X\text{ and }Y\in \cI\} $
	
\end{center}
is called the \emph{rank function} of $\cM$. The \emph{rank of $\cM$}, denoted $r(\cM)$, is $r(V)$; equivalently, the rank of $\cM$ is the size of any base of $\cM$.  
Let us remind that a set $X\subseteq V$ is independent if and only if $r(X)=|X|$. 
The \emph{closure} of a set $X$ is the set $\cl(X)=\{v\in V\colon r(X\cup\{v\})=r(X)\}$.
The matroid $\cM'=(V\setminus X,\cI')$, where $\cI'=\{Y\in \cI\colon Y\subseteq V\setminus X\}$, is said to be obtained from $\cM$ by the \emph{deletion} of $X$. The \emph{restriction}  of $\cM$ to $X\subseteq V$ is the matroid obtained from $\cM$ by the deletion of $V\setminus X$.  
If $X$ is an independent set then the matroid $\cM''=(V\setminus X,\cI'')$, where 
$\cI''=\{Y\subseteq V\setminus X \colon Y\cup X\in\cI\}$, is the \emph{contraction} of  $\cM$ by $X$. 
For a positive integer $k$, the \emph{$k$-truncation} of $\cM=(V,\cI)$ is the matroid $\cM'$ with the same ground set $V$ such that $X\subseteq V$ is independent in $\cM'$ if and only if $X\in \cI$ and $|X|\leq k$. Because in \probmwcut, we are interested only in independent sets of size at most $k$, we assume throughout our paper that the rank of the input matroids is upper bounded by $k$. Otherwise, we replace $\cM$ by its $k$-truncation. 

In our paper,   we assume in the majority of our algorithmic results that the input matroids in instances of \probmwcut are given by independence oracles. An \emph{independence oracle} for $\cM$ takes as its input a set $X\subseteq V$ and correctly returns either {\sf yes} or {\sf no}  in unit time depending on whether  $X$ is independent or not. 
We assume that the memory used to store oracles does not contribute to the input size; this is important for our kernelization results. 
Notice that given an independence oracle, we can greedily construct an inclusion-maximal independent subset of $X$ and this can be done in $\Oh(|X|)$ time.  Note also that the oracle for $\cM$ can be trivially transformed to an oracle for the $k$-truncation of $\cM$.

The \emph{partition} matroid for a given partition $\{V_1,\ldots,V_\ell\}$ of $V$ is the matroid with the ground set $V$ such that a set $X\subseteq V$ is independent if and only if $|X\cap V_i|\leq 1$ for each $i\in\{1,\ldots,\ell\}$ (in a more general setting, it is required that $|V\cap X_i|\leq d_i$ where $d_1,\ldots,d_\ell$ are some constant but we only consider the case $d_1=\dots=d_\ell=1$). 

\begin{definition}[Representative Sets]
	{\em 	Let $ \mathcal{A} $ be a family of sets of size $ p $. A subfamily $ \mathcal{A}' \subseteq  \mathcal{A}  $ is said to be $ q $-represent $ \mathcal{A} $ if for every set $ B $ of size $ q $ such that there is an $ A \in  \mathcal{A} $ that is disjoint from $ B $, there is an $ A' \in  \mathcal{A}' $ that also is disjoint from $ B $. If $ \mathcal{A}' $ $ q $-represents $ \mathcal{A} $, we say $ \mathcal{A}' \subseteq^q_{\text{rep}} \mathcal{A}$.}
	
\end{definition}

Trivially, the family $ \mathcal{A} $ itself $ q $-represents $ \mathcal{A} $. Most interestingly, it is known that for every family $ \mathcal{A} $ of sets of size $ p $ there is a subfamily $ \mathcal{A}' \subseteq^q_{\text{rep}} \mathcal{A}$ of size at most $\binom{ p+q}{q}$.

% Let  $ \M = (U, \mathcal{F}) $ be  a matroid. For a pair of sets $ A, B \subseteq U $,  we say A {\em fits}  with $ B $ if $ A $ is disjoint from $ B $ and $ A \cup B \in  \mathcal{F}$.






Matroids also could be given by their representations. Let  $\cM=(V,\cI)$ be a matroid and let $\mathbb{F}$ be a field. An $r\times n$-matrix $A$ is a \emph{representation of $\cM$ over $\mathbb{F}$} if there is a bijective correspondence $f$ between $V$ and the set of columns of $A$ such that for every $X\subseteq V$, $X\in \cI$ if and only if the set of columns $f(X)$ consists of linearly independent vectors of $\mathbb{F}^r$. Equivalently, $A$ is a representation of $M$ if $M$ is isomorphic to the \emph{column} matroid of $A$, that is, the matroid whose ground set is the set of columns of the matrix and the independence of a set of columns is defined as the linear independence.   
If $\cM$ has a  such a representation, then $\cM$ is \emph{representable} over $\mathbb{F}$ and it is also said
$M$ is a \emph{linear} (or \emph{$\mathbb{F}$-linear}) matroid. 

\begin{definition}[Representative Sets on Matroid]
	{\em 	Let $\cM=(V,\cI)$ be a matroid and let $\mathcal{S}$ be a family of subsets of $V$. For a positive integer $q$, a subfamily $\widehat{\mathcal{S}}$ is \emph{$q$-representative for $\mathcal{S}$}  if the following holds: for every set $Y\subseteq V$ of size at most $q$, if there is a set $X\in\mathcal{S}$ disjoint from $Y$ with $X\cup Y\in \cI$ then there is $\widehat{X}\in\widehat{\mathcal{S}}$ disjoint from $Y$ with $\widehat{X}\cup Y\in \cI$. }
	
\end{definition}


We write $\widehat{\mathcal{S}}\subseteq_{rep}^q\mathcal{S}$ to denote that $\widehat{\mathcal{S}}\subseteq\mathcal{S}$ is  $q$-representative for $S$. 
We use the results of of Fomin et al.~\cite{FominLPS16} to compute representative families for linear matroids. A family of sets $\mathcal{S}$ is said to be a \emph{$p$-family} for an integer $p\geq 0$ if $|S|=p$ for every $S\in\mathcal{S}$, and we use $\|A\|$ to denote the bit-length of the encoding of a matrix $A$.

\begin{proposition}[{\cite[Theorem 3.8]{FominLPS16}}]\label{prop:rep-rand}
	Let  $M=(V,\mathcal{I})$ be a linear matroid and let $\mathcal{S}=\{S_1,\ldots,S_t\}$ be a $p$-family of independent sets. Then there exists    $\widehat{\mathcal{S}}\subseteq_{rep}^q\mathcal{S}$ of size at most $\binom{p+q}{p}$. Furthermore, given a representation $A$ of $M$ over a field $\mathbb{F}$, there is a randomized Monte Carlo algorithm computing  $\widehat{\mathcal{S}}\subseteq_{rep}^q\mathcal{S}$ of size at most $\binom{p+q}{p}$ in $\mathcal{O}(\binom{p+q}{p}tp^\omega+t\binom{p+q}{q}^{\omega-1})+\|A\|^{\mathcal{O}(1)}$ operations over $\mathbb{F}$, where 
	$\omega$ is the exponent of matrix multiplication.\footnote{The currently best value is $\omega\approx 2.3728596$~\cite{AlmanW21}.}
\end{proposition}


% \subsection{Idea for Multiway Cut}


% \paragraph{Idea}

% \begin{enumerate}
% 	\item Find a normal separator (multiway cut) of size $k$.
	
% 	\item Define good and bad Configuration.
	
% 	\item Poor Scenario: Where there is a terminal component that can contain all solution vertices. Here we can not branch as parameter size remains same. It happens when we have configuration bad.
	
% 	\item Well Scenario: When no terminal component contain all solution vertices because in this case we can branch on the terminal components where $k$ strictly decrases. 
	
	
	
% 	\item We try  to go to poor scenario towards well scenario with pushing method.
	
% 	\item Pushing: Find a separtor in large component assuming it contains all the solution vertices.
	
% 	\item When no pushing method can be applicable and and we are in good configuration. We branch over terminal components. As pushing not applicable $k$ strictly decreases.
	
% 	\item Define strong separator: which creats well scenario.
	
% 	\item Once we find a strong separator, we consider this in the original graph and branch. 
% \end{enumerate}

% \newpage 

==> mwaycut.tex <==
%\newcommand{\rank}{\mathsf{rank}}

\section{Vertex Multiway Cut}\label{sec:mwaycut}

Let $G$ be a graph and $T \subseteq V(G)$ be a set of terminals. Let $S \subseteq V(G)$ be a multiway cut for $T$, and let $\cC_S$ denote the set of connected components of $G-S$. If a connected component $C \in \cC_S$ contains a terminal vertex then we call it a \emph{terminal component}; otherwise, we call it a \emph{non-terminal component}. Let $\cT_S$ denote the terminal components and $\cN_S$ denote the non-terminal components -- note that $\cC_S = \cT_S \uplus \cN_S$. We say that a $v \in S$ is adjacent to a component $C \in \cC_S$ if there exists some $u \in C$ such that $uv$ is an edge. For each $v \in S$, let $\cT(v, S) \subseteq \cT$ denote the set of terminal components that are adjacent to $v$. If the set $S$ is obvious from the context, then we denote $\cT(v, S)$ by $\cT_v$.

Consider an instance $I = (G, \cM, T, S, k)$ of \disjprob, with the following additional properties: (i) the set of connected components of $G[S]$ is exactly the vertex set of $S$, and (ii) each vertex of $S$ is adjacent to exactly one terminal component. We say that $I$ is a \emph{special instance} of \disjprob if it satisfies the following property: $I$ is a \yin of \disjprob iff there exists a solution $X$ for \disjprob, where $X$ can be partitioned into non-empty subsets $X_1, X_2$ such that, (1) $X_1$ separates some $s \in S$ from some $t \in T$, where $t$ belongs to the terminal component adjacent to $t$ (observe that, this also implies that $X_1$ separates $t$ from $T \setminus \LR{t}$), and (2) $X_2$ is a multiway cut for $T \setminus \LR{t}$.

\subsection{A Recursive Algorithm for Multiway Cut} 
\todo[inline]{idea: Correctness is \mwcut returns \textsc{yes} iff either $(G, \cM, T, k)$ is a yes-instance or $\Omega$ is a yes-instance in a specific manner (but exactly how? We need some separator. What if we cannot find that separator? Do we need it from previous call?). Initially we put $\Omega$ as a trivial no-instance like $\bot$.}

Our main algorithm is a recursive algorithm called \mwcut that takes the following as an input.
\begin{itemize}
	\item A framework $(G, \cM)$, where $G = (V, E)$ and $\cM = (V, \cI)$ on $n$ vertices,
	\item A set $T \subseteq V(G)$ of terminals, 
	\item A non-negative integer $k$,
	\item $\Omega = (G_\old, \cM_\old, T_\old, S_\old, k_\old)$ is a special instance of \disjprob. This will be useful to ``undo'' certain operations. 
 %A framework $(G_\old, \cM_\old)$, a set $T_{\old} \subseteq V(G_\old)$ of terminals, a non-negative integer $k_\old \ge 0$, and a set $S_\old \subseteq V(G_\old)$ that is a multiway cut for $T_{\old}$ in $G_{\old}$ with $|S_{\old}| \le k_{old}$, and the connected components of $G_{\old}[S_{\old}]$ are exactly the vertex set $S_{\old}$. \red{The property is that, $(G_{\old}, \cM_{\old}, T_{\old}, k)$ is a \yin iff there exists a solution $X_{\old} = X_1 \uplus X_2 \in V(G_{\old})$ such that: (i) $X_1 \neq \emptyset$ separates some $s_i \in S_\old$ from some $t_i \in T_{\old}$, and (ii) $X_1 \neq \emptyset$   }These are the \emph{old} versions of the respective objects, which will be useful to ``undo'' certain operations. Since these old versions of the objects are only required at a few specific steps in the algorithm, we abbreviate them by $\Omega$.
\end{itemize}

Given this input, the algorithm \mwcut performs the following steps. In this algorithm, whenever we conclude that the given input corresponds to a \textsc{No}-instance, we instead jump to \hyperref[step:jump]{Step 3}, where we make a call to another recursive algorithm called \dividestep, which performs some ``undo'' operations and attempts to solve the problem on $\Omega = (G_\old, \cM_\old, T_\old, k_\old)$ using divide-and-conquer. Thus, each ``jump to \hyperref[step:jump]{Step 3}'' operation should be equated to ``conclude that $(G, \cM, T, k)$ is a no-instance'' in the following.

\begin{description}[leftmargin=7pt]
	\item[Step 0: Preprocessing. \label{step:prepocess}] We perform the following preprocessing steps, the soundness of which is immediate.
	\begin{description}[leftmargin=3pt]
		\item[Rule 0.a.\label{step:disconnterm}] If there exists a terminal $t \in T$ that is disconnected from all other terminals in $T\setminus \LR{t}$ in $G$, then make a recursive call  \mwcut$(G - t, \cM - t, T - t, k, \Omega)$. 
		\\If the recursive call returns \textsc{No}, then go to \hyperref[step:jump]{Step 3}. Otherwise, return the solution returned by the recursive call.
		
		\item[Rule 0.b.\label{step:negativek}] If $k < 0$, then go to \hyperref[step:jump]{Step 3}.
	\end{description}
	
	\item[Step 1: Finding a Vertex Multiway Cut.\label{step:normalsol}] We use a known \fpt algorithm to check whether $(G, T, k)$ is a \textsc{Yes}-instance of \textsc{Vertex Multiway Cut}. Either this algorithm returns a (wlog minimal) solution $S \subseteq V(G)$ of size at most $k$ such that $G-S$ disconnects every pair of terminals, or it returns \textsc{No}. In the former case, we proceed to the next step, i.e., \hyperref[step:guessintersection]{Step 2}. In the latter case, we jump to \hyperref[step:jump]{Step 3}. Clearly, if $G$ does not admit a $k$-sized vertex cut that separates $T$, then it also does not admit an independent vertex cut. This shows the soundness of jumping to \hyperref[step:jump]{Step 3}.
	
	\item[Step 2: Branching on the intersection.\label{step:guessintersection}] If the given input is a \textsc{Yes}-instance, then it admits a solution $O \in \cI$. In this step, we try to guess the intersection $O \cap S =: Y^*$ \todo{it should by $Y$}. More specifically, we do the following: 
	\\For each $\emptyset \subseteq Y \subseteq S$, such that $Y \in \cI$, we perform the following branching. We return \textsc{Yes} iff at least one of the at most $2^k$ calls return \textsc{Yes}. Otherwise, we jump to \hyperref[step:jump]{Step 3}.
	\\\bolden{If $ Y = \emptyset$}, then we call \handlebadcut$(G, \cM, T, k, S, \Omega)$. %It either returns a solution $X$ or some $\Omega'$.
	\\\bolden{If $Y \neq \emptyset$}, then we make a recursive call to \mwcut$(G', \cM', k', \Omega)$, where $G' \coloneqq G - Y$, $\cM' \coloneqq \cM / Y$, and $k' \coloneqq k - |Y|$. 
	\begin{lemma} \label{lem:branching-soundness}
		Branching is sound and the algorithm runs in \fpt time.
	\end{lemma}
	\begin{proof}
		\red{\handlebadcut Lemma} \todo{which lemma -- todo, not written yet} proves that \handlebadcut runs in FPT time. In all other recursive calls to \mwcut, the parameter $k$ decreases by at least $1$, and thus the running time follows via induction. If $(G, \cM, T, k)$ is a \textsc{Yes}-instance, then the branch corresponding to $Y^*$ will correctly return \textsc{Yes}, which follows from induction and \red{\handlebadcut Lemma}. Otherwise, the algorithm will return \textsc{No}.
	\end{proof}
	
	
	\item[Step 3: Solving $\Omega$.\label{step:jump}] Call \dividestep on the input $\Omega = (G_\old, \cM_\old, T_\old, k_\old, )$.  We need some separator here, which one is that? From previous call?
\end{description}
This finishes the description of \mwcut.

\subsection{Disjoint Multiway Cut} 
We describe \handlebadcut on instance $I = (G, \cM, T, k, S, \Omega)$, where the goal is to find $X \subseteq V(G)$ such that
\begin{itemize}
	\item $|X| \le k$,
	\item $X$ is an independent set in $\cM$,
	\item $X$ is a \emph{multiway cut} for the terminal set $T$, and
	\item $X \cap S = \emptyset$.
\end{itemize}
If $I$ is a \textsc{Yes}-instance of \disjprob, then there exists a solution $O \subseteq V(G)$ such that $O \in \cI$ and $O \cap S = \emptyset$. For the rest of the discussion, we fix one such a solution $O$ if $I$ is a yes-instance. Naturally, this is only used in the analysis and is not needed in the algorithm.

\begin{description}[leftmargin=0pt]
	\item[Step 1: Updating the Matroid. \label{step:disjointzero}]\ 
	\\Since we are looking for a solution that is disjoint from $S$, the correctness of the following step is immediate.
	\\Remove all independent sets from $\cI$ that have a non-empty intersection with $S$. With a slight abuse of the notation, we continue to use $\cM = (V, \cI)$ to refer to the resulting matroid. Note that given a matrix representation of $\cM$, this step can be achieved by making all columns corresponding to the vertices of $S$ into the zero vector of the underlying field.
	\item[Step 2: Contracting the connected components of $S$.\label{step:contractS}]\  
	\\Recall that are required to find a solution disjoint from $S$. Let $S_1, S_2, \ldots, S_q$ denote the partition of $S$ such that each $S_i$ corresponds to a connected component of $G[S]$. We contract each $S_i$, $1\le i \le q$ into a single vertex $s_i$. Let $S' = \LR{s_1, \ldots, s_q}$. Note that $q = |S'| \le |S| \le k$. 
	
	Let $G'$ be the resulting graph. We obtain the representation of the resulting matroid $\cM'$ by removing for each $1 \le i \le q$, the zero vectors corresponding to the vertices of $S_i$ and adding a zero vector corresponding to $s_i$. Note that for any path in $G$ that visits a vertex of $v \in S_i$, there exists a path in $G'$ that uses the vertex $s'_i$, and vice versa. Further, we are still looking for a solution that avoids the vertices of $S'$. 
	
	\begin{observation} \label{obs:componentprops}
		Each terminal component contains exactly one terminal of $T$.
	\end{observation}
	\begin{proof}
		$S$ is a multiway cut for $T$, which implies that each connected component of $G-S$ contains at most one terminal of $\cT$. Further, the contraction of the connected components of $G[S]$ into single vertices does not change this fact.
	\end{proof}
	For the sake of notational simplicity, we will slightly abuse the notation and use $G, \cM, S$ to refer to $G', \cM', S'$ respectively. Further, we will use $I = (G, \cM, T, k, S)$ to be the resulting instance obtained after contraction. 
	
	\item[Step 3: Bounding the number of terminals.\label{step:largeterms}]\  
	\\If there exists a vertex $s_i \in S$ that is adjacent to at least $k+2$ distinct terminal components, then return \textsc{No}.
	\begin{lemma} \label{lem:largetermsbound}
		If there exists a vertex $s_i \in S$ that is adjacent to at least $k+2$ distinct terminal components, then $(G, \cM, T, S, k)$ is a \nin of \disjprob.
	\end{lemma}
	\begin{proof}
		Suppose $(G, \cM, T, S, k)$ is a \yin, then let $O$ be a solution that is disjoint from $S$. Let $C_1, C_2, \ldots, C_\ell \in \cT$ denote the terminal components that are adjacent to $s_i$, with $t_1, t_2, \ldots, t_\ell$ being the corresponding terminals. Note that $\ell \ge k+2$. Since $s_i \not\in O$, there exist at least two components, say $C_1$ and $C_2$ such that $O \cap C_1 = O \cap C_2 = \emptyset$. However, this implies that $G-O$ contains a path between $t_1$ and $t_2$ via $s_i$ (since $s_i \not\in O$), which is a contradiction.
	\end{proof}
	The following Observation is immediate from \Cref{lem:largetermsbound}, \Cref{obs:componentprops}, and the fact that $|S| \le k$.
	\begin{observation} \label{obs:terminal-bound}
		If $(G, \cM, T, S, k)$ is a \yin, then each $s_i \in S$ is adjacent to at most $k+1$ terminal components. Further, $|T| = |\cT| \le k^2 + k$. 
	\end{observation}
	\item[Step 3. Checking connectivity patterns.\label{step:connpatterns}] Note that there have not been any branching steps yet, and thus the running time of the algorithm is polynomial so far. In this step, we look at how the vertices of $S$ and $T$ are connected to each other, and decide to proceed in one of the following two cases. In \hyperlink{step:caseA}{case (a)}, we make a bounded number of recursive calls such that, in each branch, the parameter (i.e., the budget) strictly decreases, since we decide to include some vertices in the solution. Alternatively, in \hyperlink{step:caseB}{case (b)}, we make a \emph{single} recursive call on a smaller graph, but the parameter remains unchanged. 
	
	
	Now we check the connectivity between the vertices of $S$ and terminal components, and proceed to either of the following two cases.
	\begin{description}[leftmargin=0pt]
		\item[Case (a). Some $v \in S$ is adjacent to two at least two terminal components.\label{step:caseA}]\
		\\Fix some $v \in S$ that is adjacent to at least two terminal components. Let $\cT_v = \LR{C_1, C_2, \ldots, C_\ell}$ be the set of terminal components that are adjacent to $v$. Note that $2 \le \ell \le k+1$ due to \Cref{obs:terminal-bound}. The proof of the following observation is analogous to that of \Cref{lem:largetermsbound}.
		\begin{observation} \label{key}
			If $(G, \cM, T, S, k)$ is a \yin of \disjprob with solution $O$, then there exists some $C_i \in \cT_v$ such that $O \cap C_i \neq \emptyset$. 
		\end{observation}
		\begin{proof}
			Suppose for contradiction that $O \cap C_i = \emptyset$ for all $C_i \in \cT_v$. Since $|\cT(v, S)| \ge 2$, let $C_1, C_2$ be two distinct terminal components in $\cT_v$ and let $t_1, t_2 \in T$ be the corresponding terminals. Since $O \cap C_1 = O \cap C_2 = O \cap \LR{v} = \emptyset$, there exists a path between $t_1$ and $t_2$ in $G - O$, which is a contradiction.
		\end{proof}
		At this point, we first ``guess'', i.e., branch on one of the components $C_i \in \cT_v$(that must have a non-empty intersection with $O$, if we have a \yin), containing a terminal $t_i \in T$. This is a $(k+1)$-way branching. 
		\\(i) We now describe the branch corresponding to a particular $C_i \in \cT_v$ containing $t_i \in T$. Let $S_i \subseteq S$ denote the subset of vertices of $S$ that are adjacent to $C_i$. Note that $v \in S_i$, which implies that $1 \le |S_i| \le k$. For each $S'_i \subseteq S_i$ such that $v \in S'_i$, we further branch in the following manner. Note that this is a $2^k$-way branching.
		\\(ii) Fix some $S'_i \subseteq S_i$ such that $v \in S'_i$. Let $G'$ be the subgraph of $G$ induced on $S_i \cup C_i$. In this subgraph, we \emph{identify} all the vertices of $S'_i$ into a single vertex, say $s$, and $(S_i \setminus S'_i) \cup \LR{t_i}$ into a single vertex, say $t$, and let $G''$ denote the resulting graph. Then, for each $\mu \le k' \le k$, we solve \textsc{Rank \stc} instance $(G'', s, t, \M', k')$, where $\mu$ is the size of the min-cut between $s$ and $t$ in $G''$, where $\cM'$ is the matroid obtained from $\cM$ by setting the vectors corresponding to $s$ and $t$ to be zero vectors. For each such call, either the algorithm returns \textsc{No}, or it returns a family $\cF'$ of $st$-cuts in $G''$ that are independent in $\cM'$, and $\cF' \subseteq^{r-k'}_{rep} \mathcal{C}$, where $\mathcal{C}$ is the set of all possible independent $st$-cuts of size $k'$ in $G''$, and $r = \rank(\cM) = \rank(\cM')$. Further, the size of each $\cF'$ is bounded by $(\log n)^{\Oh(k'^3)} \cdot 2^{\Oh(k'^5)}$. \todo{should be some function of $r$}
		
		Let $\cF$ denote the union of all families $\cF'$ obtained over all branches in (i) and (ii). Note that, $|\cF| \le (\log n)^{\Oh(k^3)} \cdot 2^{\Oh(k^5)}$ \todo{should $k$ be $r$?}. If $\cF = \emptyset$, then we return \textsc{No}. Otherwise, note that the size of each set in $\cF$ is at least the size of minimum \stc in $G''$, which is strictly positive. In this case, for each $Q \in \cF$, we make a recursive call \mwcut$(G', \cM', T, k', \Omega)$, where $G' = G - Q, \cM' = \cM / Q, k' = k-|Q|$. Note that $|Q| > 0$, thus the correctness and the bound on the running time of each recursive call follows via induction.
		
		If any of the recursive calls returns a solution, we return it. Otherwise, if all recursive calls return \textsc{No}, then we return \textsc{No}.
		
		\item[Case (b). Each $v \in S$ is adjacent to at most one terminal component.\label{step:caseB}]\ 
		\\Note that without loss of generality, we can assume that each $s_i \in S$ must have exactly one terminal component adjacent to it -- otherwise we may work with a smaller solution $S \setminus \LR{s_i}$. Thus, for each $s_i \in S$, let $C_i \in \cT$ denote the terminal component adjacent to it, and let $t_i \in C_i \cap T$ be the corresponding terminal. We obtain a new graph $G'$ by identifying \todo{define identifying operation} each pair of vertices $s_i$ and $t_i$. Each of the resulting vertices $t'_i$ becomes a new terminal, and let $T'$ denote the resulting set of new terminals. \red{We modify $\cM'$ appropriately}. If $\Omega \neq \bot$, then we leave it unchanged, except the multiway cut $S_\old$ in $\Omega$ is updated to the current solution $S$. Otherwise, if $\Omega = \bot$, then we let $G_\old \coloneqq G, T_\old \gets T, \cM_\old \gets \cM, k_\old \gets k$, and $S_\old \gets S$. Then, we make a recursive call \mwcut$(G', \cM', T, k, \Omega)$. If this recursive call returns a solution, then we return it. Otherwise, we return \textsc{No}.
  
        Note that in \textbf{case (b)}, we make a \emph{single recursive call}, and $|V(G')| < |V(G)|$, thus the correctness and running time follow via induction. 
	\end{description}
\end{description}

\subsection{Undo and Divide and Conquer}
In this section, we describe the algorithm \dividestep. Recall that we are given a special instance $I = (G, \cM, T, S, k)$ of \disjprob.
%Further, it holds that each $s \in S$ is adjacent to at most one terminal component of $G-S$. Without loss of generality, we can assume that it is adjacent to exactly one terminal component, otherwise such a vertex can be removed from $S$. Thus, for each $s_i \in S$, we let $C_i \in \cT$ be the corresponding terminal component, and let $t_i \in T \cap C_i$ be the terminal in $C_i$.

%\red{Further, we know that $(G, \cM, T, k)$ is a \yin iff at least one $s_i$ and $t_i$ pair is disconnected in the graph $G[C_i \cup \LR{s_i}]$.} Thus, we perform the following $|S|$-way branching.

For each $s \gets s_i$ and $t \gets t_i$, perform the following:
\begin{itemize}
    \item Then, for each $\mu \le k' \le k$, we solve \textsc{Rank \stc} instance $(G'', s, t, \M', k')$, where $\mu$ is the size of the min-cut between $s$ and $t$ in $G''$, where $\cM'$ is the matroid obtained from $\cM$ by setting the vectors corresponding to $s$ and $t$ to be zero vectors. For each such call, either the algorithm returns \textsc{No}, or it returns a family $\cF_{k'}$ of $st$-cuts in $G''$ that are independent in $\cM'$, and $\cF_{k'} \subseteq^{r-k'}_{rep} \mathcal{C}$, where $\mathcal{C}$ is the set of all possible independent $st$-cuts of size $k'$ in $G''$, and $r = \rank(\cM) = \rank(\cM')$. Further, the size of each $\cF_{k'}$ is bounded by $(\log n)^{\Oh(k'^3)} \cdot 2^{\Oh(k'^5)}$. \todo{should be some function of $r$} Let $\cF = \bigcup_{\mu \le k' \le k} \cF_{k'}$.
    If $\cF$ is empty, then we skip the next step and proceed to the next iteration corresponding to a vertex of $S$.
    \item Let $T' \coloneqq T \setminus \LR{t_i}$. For each $Q \in \cF$, define the following: Let $G' \coloneqq G - Q$, $\cM' \coloneqq \cM / Q$, $k' \coloneqq k - |Q|$. We make a recursive call \mwcut$(G', \cM', T', k', \Omega \gets \bot)$. If any of the recursive calls returns a solution $P$, then we return $P \cup Q$. If all the recursive calls corresponding to each $Q \in \cF$ return \textsc{No}, then we proceed to the next iteration.
\end{itemize}
If all the calls return \textsc{No}, then we return that we have a \nin.

Here, we need to solve the problem by $i$ and $k-i$ branching. The parameter drops by at least one in each branch so inductively it is correct.

==> new_mwaycut_safe.tex <==


\section{Vertex Multiway Cut}\label{sec:mwaycut}



\defproblema{\probmwcut}%
{A framework $(G,\cM)$, and a terminal set $T \subseteq V(G)$}%
{Decide whether $G$ has vertex set $S\subseteq V(G)$ that is a multiway cut for $T$ in $G$ and independent in  $\cM$.
}
Like \indstcut, we will design a recursive algorithm that solves a more general version of the problem, called \textsc{Generalized Independent Multiway Cut}, or \gindmcut~for short. To this end, for any $0 \le k \le r = \rank(\cM)$, let $\cF(T, k, G) \coloneqq \LR{S \subseteq V(G) \setminus T : |S| = k, S \in \cI, \text{ and $S$ is a minimal multiway cut for $T$}}$. An instance of \gindmcut is given by $(G, \cM, T, k)$, where $0 \le k \le r$, and the task is to find an $\cF'(T, k, G) \repset{r-k} \cF(T, k, G)$ of a bounded size.

First, in \Cref{subsec:structural}, we analyze certain structural properties of solutions of \gimc, and use it to design an \fpt algorithm to find a so-called \emph{strong separator} for the instance, or to conclude that we have a \textsc{No}-instance. Then, in \Cref{subsec:recursive}, we use such a strong separator, and use to design a recursive algorithm for \gimc, and then show its correctness and that it is \fpt in $k$. 

\subsection{Finding a ``Strong Separator'' for \gimc} \label{subsec:structural}

In this subsection, we define the notion of a ``strong separator'' and how it interacts with any minimal multiway cut. Let $G$ be a graph and $T \subseteq V(G)$ be a set of terminals. Throughout the section, we will assume that $G$ is connected. Let $S \subseteq V(G)$ be a minimal multiway cut for $T$, and let $\cC_S$ denote the set of connected components of $G-S$. 
If a connected component $C \in \cC_S$ contains a terminal vertex then we call it a \emph{terminal component}; otherwise, we call it a \emph{non-terminal component}. Let $\cT_S$ denote the terminal components and $\cN_S$ denote the non-terminal components in $G-S$ -- note that $\cC_S = \cT_S \uplus \cN_S$. We say that a $v \in S$ is adjacent to a component $C \in \cC_S$ if there exists some $u \in C$ such that $uv$ is an edge. 
For each $v \in S$, let $\cT(v, S) \subseteq \cT$ denote the set of terminal components that are adjacent to $v$. If the set $S$ is obvious from the context, then we denote $\cT(v, S)$ by $\cT_v$. Given two components $C_1$ and $C_2$ we say $C_1$ is adjacent to $C_2$ (and, vice versa) if there ia a vertex in $C_1$ which has a neighbour in $C_2$. Because such a multiway cut $S$ (with certain additional properties, as stated below) will play a central role while designing the algorithm, we will often refer to it as a \emph{separator}, which is essentidefine the synonym for \emph{multiway cut for $T$}. We now define notion of good and bad configuration corresponding to a minimal separator $S$.

\begin{definition}[Good and bad configurations]
	
	Let $G$ be a graph, $T \subseteq V(G)$ be a terminal set with $|T| \geq 3$, and $S$ be a minimal multiway cut $S$ for $T$. We refer to $\tup{G, T, S}$ as a \emph{configuration}. If there is a component $C$ in $G-S$ that is adjacent to each connected component in $G[S]$, then we say that $C$ is a \emph{large component}. We say $\tup{G, T, S}$ is a {\em bad configuration}, if (i) each component in $G[S]$ is adjacent to exactly two terminal components in $G-S$, and (ii) there is a large component \footnote{Observe that, since $|T| \ge 3$, in a bad configuration, there is exactly one large component.}. Otherwise, we say that $\tup{G, T, S}$ is a {\em good configuration}. 
\end{definition}
%\subparagraph{Good and bad Configuration.}  It is easy to verify that, since $S$ is minimal, every component of $G[S]$ is adjacent to at least two terminal components. Suppose not, then let $C_1$ be such components in $G[S]$. Observe that $S \setminus V(C_1)$ still remains a multiway cut of strictly smaller size, which contradicts the minimality of $S$.
In the following claims, we prove an important property of a good and a bad configuration, respectively.

\begin{figure}[ht!]
	\centering
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=.7\linewidth]{7.pdf}
		\label{fig:sub1}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=.7\linewidth]{6.pdf}
		
		\label{fig:sub2}
	\end{subfigure}
	\caption{Examples of good (left) and bad (right) configurations. The blue and red vertices denote the separator and terminal vertices, respectively.}\label{fig:test}
\end{figure}






\begin{claim}\label{cl:goodconfig}
	If $\tup{G,T,S}$ is a good configuration, then there is no multiway cut   that is fully contained in a terminal component in $G-S$. 
\end{claim}
\begin{claimproof}
	For a contradiction, assume that there is a multiway cut $S'$ and  a terminal component $C$ in $G-S$ such that $S' \subseteq V(C)$. We know that each component in $G[S]$ is adjacent to at least two terminal components.	
	As $\tup{G, T, S}$ is a good configuration, that means that either (i) there is a component $C_S$ in $G[S]$ such that $C_S$ is adjacent to at least three terminal components, or (ii) each component in $G[S]$ is adjacent to exactly two terminal components, but there is no large component. We analyze each case separately, and show that we arrive at a contradiction.
	
	In case (i), let $C_1, C_2, C_3$ be such three components in $G-S$ that are adjacent to the vertices of $C_S$. Among $C_1, C_2, C_3$, at most one can be $C$ -- hence at least two of them, say $C_1$, and $C_2$ must have empty intersection with the set $S'$. However, since $S' \subseteq C$, it follows that $S' \cap S =\emptyset$. This implies that, in $G-S'$, there is a path between the two terminals contained inside the components  $C_1$ and $C_2$, respectively. This is contradiction to the fact that $S'$ is a multiway cut for $T$. In case (ii), we know that each component in $G[S]$ is adjacent to exactly two terminal components, but there is no large component. Recall that $S' \subseteq V(C)$ for some terminal component $C$. By the case assumption $C$ is not a large component, which implies that there is a component $C'_S$ in $G[S]$ such that $C$ is not adjacent to $C'_S$. Also we know $C'_S$ is adjacent to at least two terminal components $C_1, C_2$, and none of them is $C$. As $S' \subseteq V(C)$ and $S \cap S' \neq \emptyset$, it follows that, in $G-S'$, there is path between two terminals contained in $C_1, C_2$, respectively, which again contradicts that $S'$ is a multiway cut for $T$. Hence, the claim follows.
\end{claimproof}


\begin{claim}\label{obs:badconfig}
	If $\tup{G, T, S}$ is a bad configuration then, except possibly the large component, no other terminal component contain a multiway cut.
\end{claim}

\begin{claimproof}
	Assume that $\tup{G, T, S}$ is a bad configuration with $C$ as large component. Suppose for the contradiction, assume that some $C_1$, distinct from $C$ is a terminal component that contains a multiway cut, say $S'$. Let $C_2$ be a terminal component (arbitrary choosen) other than $C$ and $C_1$ (note that such a component must exist since $|T| \ge 3$). As $C$ is adjacent to each component in $G[S]$, hence in $G-S'$, there is path between the two terminals that are contained in $C$ and $C_2$, respectively, which contradicts that $S'$ is a multiway cut. Hence, there is no multiway cut that is fully contained in a terminal component, in $G-S$, which is not large.
\end{claimproof}


Next, we define the notion of \typea and \typeb scenarios corresponding to a minimal separator $S$.

\begin{definition}[\typea and \typeb scenarios] \label{def:scenarios}
	Given a graph $G$, a terminal set $T \subseteq V(G)$, and a minimal multiway cut $S$,  we say   the separator $S$ creates  a {\em \typea scenario} when no terminal component in $G-S $ can contain a multiway cut of size at most $|S|$. Otherwise, we say it creates a {\em \typeb scenario}.
\end{definition}

\begin{figure}[ht!]
	\centering
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=.7\linewidth]{8.pdf}
		\label{fig:sub1}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=.7\linewidth]{6.pdf}
		
		\label{fig:sub2}
	\end{subfigure}
	\caption{Example of a \typea (left) and \typeb (right) scenario. Blue and red vertices denote separator, and terminal vertices, respectively.}
	\label{fig:test}
\end{figure}

\begin{claim}\label{obs:type}
	Given a graph $G$, a terminal set $T \subseteq V(G)$, and a minimal  multiway cut $S$ of size $p$, in $2^p \cdot  n^{\cO(1)}$ time we can check whether 	$S$ creates  an \typea scenario or not.
\end{claim}
\begin{claimproof}
	If $\tup{G, T, S}$ is a good configuration, then by \Cref{cl:goodconfig} we know that there is no multiway cut   that is fully contained in a terminal component in $G-S$. Hence, in this case $S$ creates \typea  scenario. Now, assume that $\tup{G, T, S}$ is a bad configuration. Now by \Cref{cl:goodconfig} we see that except possibly the large component no other terminal component contains a multiway cut. Now to check whether large component contain a multiway cut we do the following. Let $C$ denote the large component. We take the subgraph $G_1 \coloneqq G[S \cup V(C)]$. Let $S_1, S_2, \ldots, S_q$ denote the partition of $S$ such that each $S_i$ corresponds to a connected component of $G[S]$. In the subgraph $G_1$, we contract each $S_i$, $1\le i \le q$ into a single vertex $s_i$. Let $G_2$ be the new graph after contraction. Let  $T' = \LR{s_1, \ldots, s_q}$. Note that $q \coloneqq |S'| \le |S| \le p$. Now we check whether there exists a multiway cut of size at most $p$ in the graph $G_2$ with terminal set $T'$. If \no then we conclude that   $S$ creates  a \typea  scenario in $G$ for the terminal set $T$. Otherwise, we have \typeb scenario. The correctness of the algorithm follows from the observation that $G$ has a multiway cut of size $p$ that is fully contained in $C$, if and only if $G_2$ has multiway cut of size at most $p$ with terminal set $T'$.
\end{claimproof}

Now we define a notion of a special type of multiway cut which we refer as strong separator which we use later in our algorithmic purpose.

\begin{definition}[Strong separator] \label{def:strongseparator}
	Given a configuration $\tup{G, T, S}$, we say $S$ is {\em strong separator} if (i) $\tup{G, T, S}$ is a good configuration, or (ii) $\tup{G, T, S}$ is a bad configuration, but $S$ creates a \typea scenario.	
\end{definition}




Now we prove an important result that leads to the design of a branching algorithm.




\begin{lemma}\label{lem:strongintersect}
	Let $(G, \cM, T, p)$  be an instance of \gimc with $p\geq 2$, $|T| \ge 3$, and let $S \subseteq V$ be a strong separator of size at most $p$. There exists a polynomial-time algorithm to find a pair of terminal components in $G-S$ such that for any solution $O$, we either have $S \cap O \neq \emptyset $ or one of the components must contain at least one and at most $p-1$ vertices of $O$. 
\end{lemma}
\begin{proof}
	Assume that  $(G, \cM, T, p, q)$  be an instance of \probmwcut  and    $S \subseteq V$ be a strong separator of size at most  $p$. 	 Due to the minimality of $S$, for each vertex $v \in S$ the set $S \setminus \{v\}$ is not a separator. Fix an arbitrary $v \in S$. It follows that, there exists a pair of terminals $t_1, t_2$, contained in terminal components $T_1, T_2$ respectively, such that we have  a path $P$ connecting $t_1$ and $t_2$ in $G$ such that the path intersects exactly once which is exactly at the vertex  $v$. Furthermore, $V(P) \subseteq V(T_1) \cup V(T_2) \cup \LR{v}$.
	%Hence, we get a connected component containing $v$ in $G[S]$ which is adjacent to two terminal components, say $T_1 $ and $T_2$, where  $T_1 $ and $T_2$ denotes the terminal components in $G-S$ containing the terminal vertices $t_1$, $t_2$, respectively.  
	% Hence, we also obtain that $v$ is adjacent to $T_1$ and $T_2$.
	Since $O$ is also a multiway cut for $T$, $O \cap V(P) \neq \emptyset$, which implies that $O \cap (V(T_1) \cup V(T_2) \cup \LR{v}) \neq \emptyset$. If $v \in O$ then we are done, as in this case $S \cap O \neq \emptyset$. Otherwise, $O \subseteq V(T_1 \cup T_2)$. However, since $S$ is strong separator, we know that $O \not\subseteq V(T_1)$, and $O \not\subseteq V(T_2)$. Hence, either $1 \leq  |V(T_1) \cap O| \leq k-1$ or $1 \leq  |V(T_2) \cap O| \leq k-1$. This completes the proof.
\end{proof}

\paragraph{Finding a Strong Separator}

In this section, we show that given a graph $G$ a terminal set $T$, an integer $p$ how to find a strong separator of size at most $t$ in $2^p \cdot n^{\cO(1)}$ time. First, we use a known \fpt algorithm of Cygan et al.~\cite{CyganPPW13}---that runs in time $2^p \cdot n^{\Oh(1)}$---to check whether $G$ has a minimal multiway cut of size at most $p$. Either this algorithm returns that there is no multiway cut of size $p$, or it returns a (w.l.o.g. minimal) multiway cut $S \subseteq V(G)$ of size at most $p$. In the former case, since there is no multiway cut of size $p$, there is no strong separator of size $p$ either -- hence we return that $G$ does not have a strong separator. Otherwise, in the latter case, we proceed to find a strong separator using the minimal separator $S$ returned by the algorithm, as described below. We can have the following cases. 

\begin{description}
	\item[Case A. ($\tup{G,T, S}$ is a good configuration)] Note that we can detect this case via \Cref{cl:goodconfig} in time $2^p \cdot n^{\Oh(1)}$. In this case, we are done as per the definition of a strong separator. 
	
	\medskip 
	
	\item[Case B. ($\tup{G,T, S}$ is a bad configuration)] As we are in case of a bad configuration that means that each component in $G[S]$ is adjacent to exactly two terminal components in $G-S$, and there is a large terminal component in $G-S$, say $C_L$. Assume  that the component  $C_L$ contains the terminal $t_L$. We try to find another separator of size $p$ which is fully contained in the large component using following procedure. Let $G_1 \coloneqq G-C_L$ and $G_2 \coloneqq G[S \cup C_L]$. Now consider the graph $G_2$.  For a terminal $t \in T \setminus \{t_L\}$, let $S_t \subseteq S$ denote the set of vertices in $S$ that are reachable from $t$ in the graph $G_1$. Now for each terminal vertex $t \in T \setminus \{t_L\}$ we identify all the vertices in $S_t$ to obtain a single merged vertex $v_t$. The merging operation preserves adjacencies towards the terminal components, i.e., there was a vertex $u\in V(G_2)$ such that $u$ has a neighbour in $S_t$ if and only if $u$ and $v_t$ are neighbors in the resulting graph.  Consider a  modified graph, say $H$,  with  vertex set  $\{v_t: t \in T \setminus \{t_L\}\} \cup V(C(t_L))$. We then find another minimal multiway cut with the terminal set $T':= \{t_L\} \cup \{v_t: t \in T \setminus \{t_L\}\}$. The outcome is one of the following three possibilities: (i) the answer will be \no, or (ii) we found a separator $S_1$ such that $\tup{H, T', S_1}$ is a good configuration, or (iii) we found a separator $S_2$ such that $\tup{H, S_2, T'}$ is a bad configuration. In case (i), we return that $S$ itself is a strong separator. Otherwise, in case (ii), we return that $S_1$ is the desired strong separator. Finally, in case (iii), we repeat the same procedure on $S_2$ (identify and merge) that we did for $S$, and try to find another separator. As in every step the size of the vertex set strictly decreases, this process can run at most $n$ time. And eventually we find our desired strong separator in $G$.
\end{description}




\begin{lemma}\label{lem:strong}
	There exists an algorithm that takes an input an instance $(G, \cM, T, p)$ of \gimc, where $G$ is connected, $p\geq 2$, and $|T| \geq 3$,  and in time $2^p \cdot n^{\Oh(1)}$, either returns that $\cF(T, p, G) = \emptyset$, or returns a strong separator $S$ corresponding to the instance, and two components $C_s, C_t$ satisfying the property stated in \Cref{lem:strongintersect}. Here, $n = |V(G)|$.
\end{lemma}

From the above discussion, we obtain the following corollary.

\begin{corollary} \label{cor:strong}
	An instance $(G, \cM, T, p)$ of \gimc, where $G$ is connected, $p \ge 2$, and $|T| \ge 3$, if $\cF(T, p, G) \neq \emptyset$ then $G$ has a strong separator of size at most $p$. \todo{check red}
\end{corollary}












\subsection{A Recursive Algorithm for Multiway Cut} \label{subsec:recursive}

We design a recursive algorithm called \mwcut, that takes the following as input.
\begin{itemize}
	\item A graph $G = (V, E)$, 
    \item a set $T \subseteq V(G)$ of terminals, 
	\item a matroid $\cM = (U, \cI)$, where $V(G) \setminus T \subseteq U(\cM)$, and
	\item two non-negative integers $p$, $q$ where $p+q \leq r$. \todo{should it be equal to $r$? I don't think we make it strictly less...}
\end{itemize}
We use ${\cal J} = (G, T, \cM, p, q)$ to denote the input instance to the algorithm. Given this instance $\cJ$, our goal of algorithm \mwcut is to find $\cF'(T, p, G) \repset{q} \cF(T, p, G)$ of bounded size. For the values $p=k$ and $q=0$, the solution of the instance
$(G, \cM, T, k, 0)$ corresponding to the representative set of the entire solution of size $k$ for \probmwcut in $G$ for the terminal set $T$.


\begin{description}[leftmargin=7pt]
	
	
	
	\item[Step 0: Preprocessing \label{step:prepocess}] We perform the following preprocessing steps exhaustively in the order in which they are mentioned. The soundness of these rules is immediate.
	\begin{description}[leftmargin=3pt]
		\item[Rule 0.a.\label{step:disconnterm}] If there exists a non-terminal vertex $u \in V(G)$ that has no path to any terminal vertex in $T$, then make a recursive call  \mwcut$(G - u, \cM - u, T , p,q)$. If the recursive call returns \textsc{No}, then we return 
		\no to original instance. Otherwise, return the solution returned by the recursive call.
		
		
		\item[Rule 0.b.\label{step:disconnterm}] If there exists a terminal vertex $t \in T$ that is disconnected from all other terminals in $T\setminus \LR{t}$ in $G$, then make a recursive call  \mwcut$(G - t, \cM - t, T - t, p,q)$. If the recursive call returns \textsc{No}, then we return 
		\no to original instance. Otherwise, return the solution returned by the recursive call.

        The following observation is immediate.
        \begin{obs} \label{obs:preproc}
            After an exhaustive application of Rule \hyperref[step:disconnterm]{0.a} and \hyperref[step:disconnterm]{0.b}, each connected component of $G$ contains at least two terminals of $T$. 
        \end{obs}
        
        \item[Rule 0.c.\label{step:termnumbers}] At this point we have exhaustively applied the previous two rules. Now, if the number of connected components (each of which contains at least two terminals by \Cref{obs:preproc}) of $G$ is more than $p$, then we return \no. %there exist strictly more than $p$ connected components such that every component has at least two terminal vertices then we return \no. 
        
        
		% \item[Rule 0.c.\label{step:negativek}] If $k =1$ or $|T|=2$ then go to \hyperref[step:base]{Step 1}. Else we go to \hyperref[step:normalsol]{Step 2}.
	\end{description}

	
	
		\item[Step 1: Base Case.\label{step:base}] Here we have following two cases. 
        \\Case a: If $p=1$, then $\cF(G, T, 1)$ consists of singleton vertex-sets $\LR{v}$, such that $\LR{v} \in \cI$, and $\LR{v}$ is a multiway cut for $T$ (of size $1$). For each $v \in V(G) \setminus T$, we can easily check whether $v \in \cF(G, T, 1)$ in polynomial time; this implies that the set $\cF(G, T, 1)$ can be found in polynomial time. Then, we compute $\cF'(G, T, 1) \repset{q} \cF(G, T, 1)$ in 
        $n^{\cO(1)}$ time, and return $\cF'(G, T, 1)$. The correctness of this step is immediate.
        \\Case b: If $|T|=2$, then we solve the instance $(G, \cM, s, t, p, q)$ of \indstcut using \Cref{thm:stcuttheorem}, and return the family returned by the algorithm. The correctness of this step follows from that of \Cref{thm:stcuttheorem}, and the theorem implies that this step runs in time \red{time...} and returns a family $\cF'(G, \{s,t\}, p)$ of size \red{size...}. The correctness of this step is immediate.

        \begin{claim} \label{cl:basecase}
		Let $\cF'(G, T, p)$ denote the set that we return in the base case. Then $\cF'(G, T, p) \repset{q}  \cF(T, p, G)$.
	\end{claim}
	
	\medskip
	
	\item[Step 2: Solving the problem in a disconnected graph. \label{step:connected}] In this step, we describe how to deal with the problem when the underlying graph is not connected. Let $(G, \cM, T,p,q)$ be the instance and $G$ be the union of $\ell$ connected components $G_1, \ldots G_\ell$. Observe that after an exhaustive application of the preprocessing (\hyperref[step:prepocess]{Rule 0.b}), each component in $G$ has at least two terminal components, so each minimal solution must have a non-empty intersection with each terminal component. Hence, we can assume that $\ell \leq p$. Let $T_i := T \cap V(G_i)$. 	Now for each component $G_i$ we try to find the smallest $p_i \leq p$ such that $G_i$ has an independent multiway cut of size $p_i$ -- which can be found by making a recursive call to the algorithm for each component separately, starting from $p'_i =1, 2, \ldots, p$, in order to find the smallest value $p_i$ such that the recursive call for all $p'_i < p_i$ returned \no, and $p_i$ returns a non-empty family. Note that, assuming the number of connected components is more than $1$, if for some $i \in [\ell]$, we find that for $p'_i = p-1$, the instance $(G_i, \cM, T_i, p_i, q+p-p_i)$ is a \no-instance, then we conclude that we have a \no-instance.
    The correctness of this follows from the fact that any $S \in \cF(T, p, G)$ must have a non-empty intersection with each connected component. Hence, in each recursive call, the parameter strictly decreases. Note that we make a recursive call to most $p^2$ many sub-problems. Let $p_i$ be the smallest value for each  component $G_i$ such that we find non-empty solution for $(G_i, \cM, T_i,p_i,q+p-p_i)$. Note that the $p_i$'s form a natural partition $\cP$ of $p$ such that $p = p_1 + \ldots + p_\ell$. Let $\cF'_i$ be the output of the $i$th call with parameter $p_i$. We compute $\cF'_1 \bullet \cF'_2 \bullet \cdots \bullet \cF'_\ell$, and we filter out any sets from the resultant that do not constitute a minimal independent multiway cut of size $p$ for $T$. Let the remaining collection of sets be $\cF^1(T, p, G) $. Finally, we compute and return $\cF'(T, p, G) \repset{q} \cF^1(T, p, G)$. 
	
	\begin{claim} \label{cl:disconnected}
		$\cF'(T, p, G) \repset{q} \cF(T, p, G)$.
	\end{claim}
	\begin{claimproof}
    %If $(G, \cM, T, p, q)$ is a \no-instance, then $\cF(T, p,  G) = \emptyset$, and by induction hypothesis, we have that $\cF'_i \repset{q} \cF(T_i, p_i,  G_i)$, which implies that $\cF'_i = \emptyset$ (via \Cref{obs:repsetprops}) for some $i$, and hence $\cF'(T, p, G)  = \emptyset$, and we are done. 
    We show the claim in two parts. First, we show that $\cF'(T, p, G)\subseteq \cF(T, p, G)$, and then we show that the former also $q$-represents the latter. For the first part, consider an $R \in \cF'(T, p, G)$. Hence, for each $i \in [\ell]$, there exists some $R_i $
 

 
	Otherwise, assume that $\cF(T, p,  G) \neq \emptyset$. Let $Y \subseteq U(\cM)$ be a set of size $q$ such that there is a set $O  \in \cF(T, p,  G)$  (i.e., $O$ is a minimal multiway cut of size $p$ for $T$), such that $O $ fits $Y$.  We have to show that there is a $\hat{X}  \in \cF'(T, p, G)$, such that $\hat{X}$ fits $Y$, that is also a minimal multiway cut of size $p$ for $T$. 
	
	We know that $\cF'_i$ is the output of the recursive call on $(G_i, \cM, T_i, p_i, q+p-p_i)$. By induction (recall that $p_i < p$), we know that $\cF'_i \repset{q+p-p_i} \cF(G_i, p_i, T_i)$. 
    Let $O_i \coloneqq O \cap V(G_i)$, $Y_i \coloneqq Y \cap V(G_i)$, and $Y_{out} = Y \setminus V(G)$. Note that $Y = Y_1 \cup Y_2 \cup \ldots \cup Y_\ell \cup Y_{out}$. Now we provide a recursive definition of $\hat{X_i}$ for each $i \in [\ell]$. The set $\hat{X_1}$ is a representative for the set $O_1$ in the graph $G_1$ for the $p+q-p_1$ sized set $(O \cup Y) \setminus O_1$. Now for $i>1$ 
    $$Z_i \coloneqq \lr{\bigcup_{j<i} (\hat{X_j} \cup Y_j)} \cup Y_i \cup \lr{\bigcup_{j>i} (O_j \cup Y_j)} \cup Y_{out}.$$
	
	 Clearly, $|Z_i|= p+q-p_i$. By the property of $\cF'_i$, there exists some $\hat{X_i} \in \cF'_i$, such that $\hat{X_i} $ is a minimum multiway cut of size $p_i$ for $T_i$ in $G_i$, and $\hat{X_i}$ fits  $Z_i$. Now, let $\hat{X} \coloneqq \hat{X_1} \cup \cdots \cup \hat{X_{\ell}}$. Clearly $|\hat{X}|= \sum_{i=1}^{\ell} p_i= p$.  As $\hat{X_i}$ is a solution for $G_i$ and $G$ consists of $\ell$ components $G_i, i\in [\ell]$,  so $ \hat{X} \coloneqq \hat{X_1} \cup \cdots \cup \hat{X_{\ell}} $ is a solution for $G$. By our recursive definition, we can conclude that $\hat{X_{\ell}} \cup Z_{\ell} $ is an independent set. Since $\hat{X_{\ell}} \cup Z_{\ell} = \hat{X} \cup Y$, we are done.
	\end{claimproof}
	
	
	
%	For this case, for each partition $\cP$ of the integer $p$ into positive integers $p_1, p_2, \ldots, p_\ell$, such that $p = p_1+ \ldots+p_{\ell}$, we solve $(G_i, \cM, T_i,p_i,q+p-p_i)$ for each $i \in \ell$.  As we are finding a minimal solution, we can only focus on the components which contain at least two terminal vertices. So $\ell \leq p$.
%	
%	\todo{Add observation: First, show $\ell \le p$. Also show number of different partitions is $p^p$.}
%	
%	\red{%maybe new
%		We only have one partition $\cP$ of $p = p_1 + \ldots + p_\ell$. Then $\cF'_i$ be output of $i$th call. We compute $\cF^1(T, p, G) \coloneqq \cF'_1 \bullet \cF'_2 \bullet \cdots \bullet \cF'_\ell$. Then, we return $\cF'(T, p, G) \repset{q} \cF(T, p, G)$. 
%		
%		\begin{claim}
%			$\cF^1(T, p, G) \repset{q} \cF(T, p, G)$.
%		\end{claim}
%		\begin{proof}
%			Induction + may need to rely on generalization of \Cref{obs:repsetprops} item 3.
%		\end{proof}
%	}
%	
%	\red{Let $\cF'(i, p_i, \cP)$ be output of $i, p_i$ when partition was $\cP$. Then, for one fixed $\cP$, let $\cF^1(\cP) \coloneqq \cF'(1, p_1) \bullet \cF'(2, p_2) \bullet \cdots \bullet \cF'(\ell, p_\ell)$. Finally, let $\cF^1(T, p, G) \coloneqq \bigcup_{\cP} \cF^1(\cP)$. We will return $\cF'(T, p, G) \repset{q} \cF^1(T, p, G)$. 
%		
%		\begin{claim}
%			For a fixed partition $\cP$, $\cF^1(\cP) \repset \cF(T, p, G, \cP)$, where $\cF(T, p, G, \cP) \subseteq \cF(T, p, G)$, 
%		\end{claim}
%		
%	}
%	
	
	\medskip
	
	\item[Step 3: Finding a Strong Separator.\label{step:normalsol}] Since \hyperref[step:connected]{Step 2} is not applicable, we know that the graph $G$ is connected. Then we use our \fpt algorithm of \cref{lem:strong} to check whether $G$ has a strong separator corresponding to the instance $(G, \cM, T, p,q)$ that runs in time $2^p \cdot n^{\Oh(1)}$. Either this algorithm returns a (w.l.o.g. minimal) separator $S \subseteq V(G)$ of size at most $p$, or it returns \textsc{No}. In the former case, we proceed to the next step, i.e., \hyperref[step:guessintersection]{Step 4}. In the later case, we return \no to our original instance $(G, \cM, T, p,q)$. Because if $G$ does not admit a multiway cut for $T$ of size $p$, then it also does not admit an independent vertex multiway cut of size $p$. This shows the soundness of returning \no.
	
	\medskip
	
	
	
	\item[Step 4: Branching procedure. \label{step:guessintersection}] Let $\cF \coloneqq \cF(G, T, p)$ denote the family of feasible solutions for the given instance $\cJ = (G, \cM, T, p, q)$. If $\cF \neq \emptyset$, then \Cref{lem:strongintersect} implies that, there exists a pair of components $C_s$ and $C_t$, such that for any $O \in \cF$, for each strong separator $S$ of size $p$ corresponding to the terminal set $T$, we  have that, either (i) $S \cap O \neq \emptyset $, or (ii) either  $1 \leq  |C_s \cap O| \leq p-1$, or $1 \leq  |C_t \cap O| \leq p-1$. Furthermore, as stated in \Cref{lem:strongintersect}, given a strong separator $S$, such a pair of components can be found in polynomial-time. 
    However, since a-priori we do not know whether case (A) or (B) is applicable, we design a branching strategy that considers both possibilities. We describe this branching in the following. 
    %This leads to the following branching strategy , where we consider case (i), and (ii) respectively. 
	
	\begin{description}
		\item[Handling case (A): Branching on the vertices in $S$:] We branch on each vertex $v$ on $S$ assuming that $v \in S \cap O$.   More specifically, we do the following: For each vertex $v \in  S$ we make a recursive call to \mwcut$(G-v, \cM, T, p-1, q)$. Let $\cF'(v)$ be the set returned by the recursive call. Then $\cF^1(v) \coloneqq \cF'_v \bullet \LR{v}$. 
		
		
			
			\begin{claim} \label{cl:s-branchingrepset}
				$\cF^1(v) \repset{q} \cF(T, p, v, G)$, where $\cF(T, p, v, G) \subseteq \cF(T, p, G)$ is the set of all independent minimal multiway cuts for $T$ that contain $v$. 
			\end{claim}
			
	\begin{claimproof}
		%Recall that $\cF'(C_t, \cP, p_1) \repset{q} \cF^1(C_t, \cP, p_1) = \cF'(T_1, p_1, G_1) \bullet \cF'(T_2, p_2, G_2)$. Hence, by \Cref{obs:repsetprops} (item 1), it suffices to prove that $\cF^1(C_t, \cP, p_1) \repset{q} \cF(T, p, G, C_t, \cP, p_1)$. 
        First we argue that $\cF^1(v) \subseteq \cF(T, p, v, G)$, and then we show that $\cF^1(v)$ also $q$-represents $\cF(T, p, v, G)$. Consider some $R \in \cF^1(v)$, and $R$ must be equal to $Q \cup \LR{v}$ for some $Q \in \cF'_v$. By induction hypothesis, $Q \in \cF(G-v, T, p-1)$, i.e., $Q$ is a miminmal multiway cut for $T$ of size $p-1$ in $G-v$. It follows that $R = Q \cup \LR{v}$ is also a minimal multiway cut of size $p$ for $T$ in $G$. Since $v \in R$, this shows that $\cF^1(v) \subseteq \cF(T, p, v, G)$.
        %If $(G-v, \cM, T, p-1, q)$ is a \no-instance, then $\cF(T, p, v, G) = \emptyset$, and by induction hypothesis, we have that $\cF'_v \repset{q} \cF(T, p, v, G)$, which implies that $\cF'_v = \emptyset$ (via \Cref{obs:repsetprops}), and hence $\cF'_v = \emptyset$, and we are done. 

        Now, consider some $Y \subseteq U(\cM)$ of size $q$ for which there is a set $O  \in \cF(T, p, v, G)$  such that $Y$ fits $O$. First, by the induction hypothesis, we have $\cF'(v) \repset{q+1} \cF(T, p-1,  G-v) $. This implies, in particular, that each $X \in \cF'(v)$, is a minimal multiway cut of size $p-1$ for $T$ in $G-v$.     
        We have to show that there is a $\hat{X}  \in \cF^1(v)$, such that $\hat{X}$ is a minimal multiway cut of size $p$ in  such that $\hat{X}$ fits $Y$. 	As $\cF(T, p, v, G) \subseteq \cF(T, p, G)$ is the set of all independent minimal multiway cuts for $T$ that contain $v$, the vertex $v$ must belong to $O$. Consider the set $O_v \coloneqq O \setminus \{v\}$ and $Y_v \coloneqq Y \cup \{v\}$. Clearly $O_v \cup Y_v = O \cup Y$, and for any $X \in \cF'(v)$, $v \not\in X$.  
        %We know that $\cF'(v)$ is the set returned by recursive call of the algorithm \mwcut to the instance $(G-v, \cM, T, p-1, q+1)$. 
        %Now, by the induction hypothesis, we have $\cF'(v) \repset{q+1} \cF(T, p-1,  G-v) $. 
        So for the set $Y_v \subseteq U(\cM)$,  of size $q+1$  there is a set $O_v  \in \cF(T, p-1,  G-v)$, such that $O_v$ fits $Y_v$. Hence, there exists $X_v \in \cF'(v)$ such that $X_v$ also fits $O_v$. Further, $X_v \in \cF(T, p-1, G-v)$ as well. Now, consider the set $\hat{X} \coloneqq X_v \cup \{v\}$. Obviously, $\hat{X}$ is disjoint from $Y$. As $X_v$ is an independent multiway cut for $T$ in $G-v$, so $\hat{X} = X_v \cup \LR{v}$ is an independent multiway cut in $G$. Finally, since $\hat{X} \cup Y= X_v \cup Y_v \in \cI$, the claim follows.
	\end{claimproof}
		
		\smallskip 
		
		\item[Handling case (B): Branching on terminal components in $G-S$:] For a terminal vertex $x \in T$, we use the notation $C_x$ to denote the terminal component in $G-S$ containing the vertex $x$. Recall the components $C_s$ and $C_t$ returned by \Cref{lem:strongintersect} with the property that, if $\cJ$ is a \yes-instance, and for some $O \in \cF(T, p, G)$, it holds that $O \cap S = \emptyset$, then either $1 \le |O \cap V(C_s)| \le p-1$, or $1 \le |O \cap V(C_t)| \le p-1$.
        %This branching step takes care of the case that $S \cap O =\emptyset $. By \cref{lem:strongintersect}, we know that if  $S \cap O = \emptyset $ then there is a pair of  terminal components    such that  one of the componets has non-empty intersection with at most $(k-1)$ vertices with $O$. 
        %Let $C_t$ and $C_s$ be such components that we able to find in polynomial time (assuming we have $S$ in our hand). 
        %We know that, if $\cJ$ is a \yes-instance, then either $1 \leq |V(C_t) \cap O| \leq (k-1)$ or $1 \leq |V(C_s) \cap O| \leq (k-1)$.
        First we guess (i.e., branch) which components among $C_t$ and $C_s$ have the above mentioned property. WLOG, assume that the component $C_t$ has such property, and the other case is symmetric. 	
        
        Let $\reach(t)$ denote the set of vertices in $S$ which is reachable (connected) from the vertex $t$ in the induced subgraph $G[C_t \cup S]$.
		Next, we guess the following two things (i) the value $|V(C_t) \cap O|$ and (ii) the connectivity among the vertices in $S \cup \{t\}$ in the subgraph $G[V(C_t)  \cup \reach(t)]- O$.  More specifically,  we  guess a partition of the vertices in $\reach(t) \cup \{t\}$ such that it holds the following property: a pair of vertices $x,y \in \reach(t) \cup \{t\}$ belongs to the same set of the partition if and only if there is a path between $x$ and $y$ in $G[V(C_t)  \cup \reach(t)]- O$. We introduce the following notation.
        \begin{definition}
            Given a graph $H$ and partition $\Pi$ of vertex set $U \subseteq V(H)$, the graph obtained in the following procedure is denoted by $H^*/\Pi$: for each part $\pi \in \Pi$, we \identity all the vertices of $\pi$ into a single vertex, say $v_{\pi}$ (we refer preliminary section to detail about the \identity operation). 
        \end{definition}
        
        Now in our algorithm,  for the  component $C_t$,  for each partition  $\cP$ of the vertex set $ \reach(t) \cup \LR{t}$, for each integer $1 \le p_1 \le p-1$ (let $p_2 = p-p_1$),
        %, assuming $T^*$ is the new terminal set 
        we create two instances of \probmwcut and recursively call \mwcut on each of them. We highlight that the parameters for both the instances satisfy $1 \le p_1, p_2 \le p-1$, hence the parameter strictly decreases in both the recursive calls. These two instances are defined as follows. \todo{add figure}
		\smallskip 
		
		\begin{itemize}[leftmargin=2pt]
			\item Instance 1 is $\cJ_1 \coloneqq (G_1, \cM, T_1, p_1, q+p_2)$. Here $G_1$ is $H^*/\cP$, where $H:= G[V(C_t)  \cup \reach(t)]$. That is  $V(G_1) = V(C_t) \cup V(\cP)$ where $V(\cP)$ is the set of all new vertices added after processing \identity operation on each $P \in \cP$. And the terminal set $T_1:= V(\cP)$. Let $\cF'(T_1, p_1, G_1) \repset{q+p_2} \cF(T_1, p_1, G_1)$ is the output returned by recursive call. 
            By induction this is true. 
			
			\item Instance 2 is $\cJ_2 \coloneqq (G_2, \cM, T_2, p_2, q+p_1)$. Here, the description of the graph $G_2$ and terminal set $T_2$ is based on the partition $\cP$.  We have the following two cases depending on whether the vertex $t$ is identified with some other vertices in $\reach(t)$ in $\cP$ or not. Let $P_t$ denotes the set in the partition in $\cP$ which contains $t$.
			
			\begin{description}[leftmargin=3pt]
				\item[Case 4.a. $|P_t|=1$  \label{case:t=0}] Here $t$ is not in same part in $\cP$ with any $v \in \reach(t)$. Note that this implies that we require that $t$ is disconnected from all $v \in \reach(t)$ in each solution of $\cJ_1$. Since any path between $t$ and $t'$ in $G$ must use a vertex of $\reach(t)$, it follows that $G - X$ already disconnects $t$ from all $t' \in T\setminus \LR{t}$, for any solution $X$ of $\cJ_1$. Hence, in $\cJ_2$, we may remove $t$ from $T$.
                \\More formally, we define $G_2 \coloneqq G^*/\cP- V(C_t)$, and $T_2 \coloneqq T \setminus \{t\}$. That is,  $V(G_2) = \big(V(G) \setminus \large(V(C_t) \cup \reach(t))\big) \cup \big(V(\cP) \setminus \LR{t}\big)$. 
				
				\smallskip 
				
				
				
				\item[Case 4.b. $|P_t|\geq 2$  \label{case:t=1}] In this case, the terminal $t$ is identified with at least one vertex from $\reach(t)$. Let $v_t$ denote the result of the \identity operation on the set $P_t$.
                \\In this case $G_2 \coloneqq G^*/\cP- (V(C_t)\setminus \{t\})$, and $T_2 \coloneqq T \setminus \{t\} \cup \{v_t\}$. That is  	$V(G_2) = \lr{V(G) \setminus \lr{V(C_t) \cup \reach(t)}} \cup V(\cP)$. 
                \\Let $\cF'(T_2, p_2, G_2) \repset{q+p_1} \cF(T_2, p_2, G_2)$ is the output returned by recursive call. By induction this is true. 
				
				
			\end{description}
		More formally, let ${\cal G}_t$ as the collection of all tuples $(C_t, \cP, p_1)$ of guesses corresponding to component $C_t$ -- analogously, we also define the set of guesses corresponding to $C_s$, and also recursively call the algorithm on each pair sub-instances (we omit this description).
  
 		Now to return the solution for branching on terminal components, we do the following. First we compute $ \cF'(T_1, p_1, G_1) \bullet \cF'(T_2, p_2, G_2)$, and from the resultant, we filter out any sets that do not form an independent minimal multiway cut for $T$ in $G$. Let us refer to the remaining $p$-family as $\cF^1(C_t, \cP, p_1)$. 
    %Then we compute  $\cF'(C_t, \cP, p_1) \repset{q} \cF^1(C_t, \cP, p_1)$. 
    We say a minimal independent multiway cut $O$ is {\em compatible} with the guess $(C_t, \cP, p_1)$ if following two conditions hold: (i) $|O \cap V(C_t)|=p_1$, (ii) for any pair of vertices $u,v \in \reach(t) \cup \{t\}$, if $u$ and $v$ belong to  two different sets in the partition $\cP$, then there is no path from $u$ to $v$ in the subgraph $G[V(C_t) \cup \reach(t) \setminus O]$.
				
				\begin{claim} \label{cl:divide}
					$\cF^1(C_t, \cP, p_1) \repset{q} \cF(T, p, G, C_t, \cP, p_1)$, where $\cF(T, p, G, C_t, \cP, p_1) \subseteq \cF(T, p, G)$ is the set of minimal independent multiway cuts that are compatible with the guess $(C_t, \cP, p_1)$. 
				\end{claim}
			
			\begin{proof}
            %Recall that $\cF'(C_t, \cP, p_1) \repset{q} \cF^1(C_t, \cP, p_1) = \cF'(T_1, p_1, G_1) \bullet \cF'(T_2, p_2, G_2)$. Hence, by \Cref{obs:repsetprops} (item 1), it suffices to prove that $\cF^1(C_t, \cP, p_1) \repset{q} \cF(T, p, G, C_t, \cP, p_1)$. 
            First, we show that $\cF^1(C_t, \cP, p_1) \subseteq \cF(T, p, G, C_t, \cP, p_1)$. To this end, consider any $R \in \cF^1(C_t, \cP, p_1)$, which implies that there exists some $P \in \cF'(T_1, p_1, G_1), Q \in \cF'(T_2, p_2, G_2)$, such that $R = P \cup Q$, $P \cap Q = \emptyset$, and $R$ is indeed a minimal multiway cut of size $p$ for $T$ in $G$. Firstly, note $R \cap V(C_t) = P$, which implies that $|R \cap V(C_t)| = |P| = p_1$. Secondly, since $P \in \cF'(T_1, p_1, G_1) \repset{q+p_2} \cF(T_1, p_1, G_1)$, it follows that, for any $u, v \in \reach(t) \cup \LR{t}$, such that $u, v$ belong to different parts of $\cP$, there is no path from $u$ to $v$ in $G_1 - P$. Therefore, there is no path from $u$ to $v$ in $G[(V(C_t) \cup \reach(t))] - P = G[(V(C_t) \cup \reach(t)) \setminus R]$. This shows that $R$ is indeed compatible with the guess $(C_t, \cP, p_1)$, i.e., $R \in \cF(T, p, G, C_t, \cP, p_1)$. 
            
           %If $(G, \cM, T, p, q)$ is a \no-instance, then $\cF(T, p,  G) = \emptyset$, and by induction hypothesis, either $\cF(T_1, p_1, G_1) = \emptyset$ or $\cF(T_2, p_2, G_2) = \emptyset$. As we have that $\cF'(T_i, p_i, G_i) \repset{q+p-p_i} \cF(T_i, p_i,  G_i)$, which implies that $\cF'(T_i, p_i, G_i) = \emptyset$  (via \Cref{obs:repsetprops}) for some $i$, and hence $\cF^1(C_t, \cP, p_1)  = \emptyset$ that indeed apply $\cF^1(C_t, \cP, p_1)  = \emptyset$ (via \Cref{obs:repsetprops}), and we are done. 
            %Otherwise, assume that $\cF(T, p,  G) \neq \emptyset$.				Let $Y \subseteq U(\cM)$ be a set of size $q$ such that there is a set $O  \in \cF(T, p, G, C_1, \cP, p_1)$. That is,  $O$ is a minimal multiway cut of size $p$ for $T$ that is compatible with the guess $(C_t, \cP, p_1)$, and $O $ fits $Y$.  We have to show that there is a $\hat{X}  \in \cF'(C_t, \cP, p_1)$, such that (i) $\hat{X}$ fits $Y$, and (ii) $\hat{X}$ is also a minimal multiway cut of size $p$ for $T$.

            Next, we show that $\cF^1(C_t, \cP, p_1)$ also $q$-represents $\cF(T, p, G, C_t, \cP, p_1)$. To this end, consider $Y \subseteq U(\cM)$ of size $q$, for which there exists some $O  \in \cF(T, p, G, C_1, \cP, p_1)$ such that $O$ fits $Y$. We show that there exists some $\hat{X} \in \cF^1(C_t, \cP, p_1)$ such that $\hat{X}$ also fits $Y$.    
            %We know that for each $i \in \{1,2\}$, $ \cF'(T_i, p_i, G_i) $ is the output of the recursive call on $(G_i, \cM, T_i, p_i, q+p-p_i)$. 
            Let $O_i \coloneqq O \cap V(G_i)$, $Y_i \coloneqq Y \cap V(G_i)$, and $Y_{out} \coloneqq Y \setminus V(G)$. Note that $Y = Y_1 \cup Y_2 \cup Y_{out}$. Now we define the set $\hat{X_i}$ for each $i \in [2]$. The set $\hat{X_1}$ is a representative for the set $O_1$ in the graph $G_1$ for the $q+p_2$ sized set $(O \cup Y) \setminus O_1$. Let  $X_2= \hat{X_1} \cup Y$. As $|X_2|= q+p_1$ by induction, there exists some $\hat{X_2} \in \cF'(T_2, p_2, G_2)$, such that $\hat{X_2} $ is a minimum multiway cut of size $p_2$ for $T_2$ in $G_2$, and $\hat{X_2}$ fits  $O_2$.
				 Now, let $\hat{X} \coloneqq \hat{X_1} \cup  \hat{X_2}$. Clearly $|\hat{X}|= |\hat{X_1}| +  |\hat{X_2}|= p_1 + p_2$.  By our argument, we can conclude that $\hat{X_{2}} \cup X_{2} $ is an independent set. Since $\hat{X_{2}} \cup X_{2} =\hat{X_{2}} \cup \hat{X_1} \cup Y = \hat{X} \cup Y$, we have that $\hat{X} \cup Y$ is an independent set. 
     
                It remains to show that $ \hat{X} $ is a minimal multiway cut for $T$ in $G$. Consider a shortest path $P_{12}$ between two terminal vertices, say $t_1, t_2 \in T$ in $G-\hat{X}$.
                
                
                \begin{description}
                    \item[Case 1] First, we analyze the case where $t \notin \{t_1, t_2\}$. Naturally, $P_{12}$ is also a shortest path between $t_1$ and $t_2$. In this case, the path $P_{12}$  must use a vertex from $V(C_t)$, otherwise $\hat{X_2}$ is not a solution for $\cJ_1$. We first claim that, $|V(P_{12}) \cap \reach(t)| \ge 2$. Suppose to the contrary that $|V(P_{12} \cap \reach(t)| \le 1$, then there exists a path $P'_{12}$ in $G_2 - \hat{X}_2$ between $t_1$ and $t_2$, which contradicts that $\hat{X}_2$ is a solution for $\cJ_2$. Thus, $|V(P_{12}) \cap \reach(t)| \ge 2$, Now consider distinct $x_1, x_2 \in V(P_{12}) \cap \reach(t)$, such that the internal vertices of the subpath $P'_{12}$, say $I$, between $x_1$ and $x_2$ satisfies that $\emptyset \neq I \subseteq V(C_t)$. 
                    %First, note that $t \notin I$ -- otherwise we obtain a path between $t$ and $t_1$ (or $t$ and $t_2$) that is shorter than $P_{12}$, a contradiction. 
                    Now, suppose that
                    $x_1$ and $x_2$ are adjacent in $G$, then we can obtain a path between $t_1$ and $t_2$  by replacing $x_1, V(I), x_2$ by the edge $x_1x_2$ in $P_{12}$, which yields a shorter path between $t_1$ and $t_2$, which is a contradiction to the assumption that $P_{12}$ is a shortest path. To summarize, we have a subpath $P'_{12}$ of $P_{12}$ such that the endpoints of $P'_{12}$, i.e., $x_1, x_2 \in \reach(t)$, and $\emptyset\neq I \subseteq V(C_t)$. Now we consider different cases, and arrive at a contradiction.
                \\Case (1a): 
                 $x_1$ and $x_2$ are in the same part $P \in \cP$. Then, $P$ is contracted into a single vertex $v_P$ in $G_2$. This implies that there is a path between $t_1$ and $t_2$ in $G_2-\hat{X}_2$ as well, which is a contradiction.
                 %(i) If $t \in P$ as well (as in Case 4b), then it follows that, in $G_2-\hat{X}_2$, there is a path from $t$ to $t_1$ (or from $t$ to $t_2$), which contradicts the assumption that $\hat{X}_2$ is a solution for $\cJ_2$. (ii) If $t \not\in P$ (as in Case 4a), then since $P$ is identified into a single vertex in $G_2$, it follows that there is a path between $t_1$ and $t_2$ in $G_2 - \hat{X}_2$ as well, which is again a contradiction.
                 \\Case (1b): $x_1$ and $x_2$ are in different parts $P_1$ and $P_2$ respectively, which are identified into the vertices $v_1, v_2$ in $G_1$, respectively. However, this implies that there is a path $P'_{12}$ between $v_1$ and $v_2$ in $G_1-\hat{X}_1$, which contradicts that $X_1$ is a solution for $\cJ_1$.
                 %Now, we note that is a path between $x_1$ and $x_2$ in $G[V(C_t) \cup \reach(t)] - \hat{X_1}$, it contradicts the assumtion that $ \hat{X_1} $ is a solution for $(G_1, T_1, p_1)$.


                \item[Case 2] Now, we analyze the case where $t \in \{t_1, t_2\}$. W.l.o.g., assume that $t=t_1$; hence $P_{12}$ is a shortest path between $t$ and $t_2$ in $G-\hat{X}$.        
                In this case, as $t \in V(C_t)$ the path $P_{12}$  must use a  vertex from $(V(C_t) \setminus \{t\}) \cup \reach(t)$.  In path $P_{12}$, let $x_2$ denote the vertex in $\reach(t)$ such that all the internal vertices of the subpath connecting $x_2$ to $t$ along $P_{2}$ are from $V(C_t)$. Now we consider different cases and arrive at a contradiction.  \\Case (2a): 
                 $x_2$ and $t$ are in the same part $P \in \cP$.  Then it follows that there is a path from $t_2$ to $v_P$ in $G - \hat{X_2}$, which contradicts the assumption that $ \hat{X_2} $ is a solution for $\cJ_2$.
                            \\Case (2b): $t$ and $x_2$ are in different parts. Now, we note that there is a path between $t$ and $x_2$ in             $G[V(C_t) \cup \reach(t)] - \hat{X_1}$, it contradicts the assumption that $ \hat{X_1} $ is a solution for $\cJ_1$.
                                
                \end{description}
                
                              
                This completes the claim. \todo{add figure}
			\end{proof}

   Here is a simple observation.

   \begin{claim}\label{claim:compatible}
       Consider any $O \in \cF(T, p, G)$ such that $O \cap S = \emptyset$. Then, there is some guess $(C_t, \cP, p_1)$ with which  $O$ is compatible.
       
   \end{claim}  
 

   \begin{claimproof}
  Assuming that $O \cap S = \emptyset$, we know that at least one of the components $C_s$ or $C_t$ has non-empty intersection with the vertices of  $O$. Now we obtain a guess which is compatible with $O$. Assume  that $|V(C_t) \cap O|=p_1 > 0$.  Let $\cP$ be the partition of the vertices in $\reach(t) \cup \{t\}$ defined by as follows. A pair of vertices $u$ and $v$ from $\reach(t) \cup \{t\}$ belongs to different part if they are not connected in the graph $G[V[C_t] \cup \reach(t)] - O$ as well as the graph $G- (V(C_t) \cup O)$. It is easy to see that guess $(C_t, \cP, p_1)$ is comatible with $O$.
   \end{claimproof}
			
			
		\end{itemize} 
		
		
		
		
		
		
		
		
		
		
		
		
		
		
	\end{description}  
	
	
	\medskip 
	
	\item[Step 5: Return as output] We return \textsc{no} if each of the branching steps returns \no to their corresponding instance. Otherwise, we do the following.
	Notice that in each branching step, we have at most $p+ 2(p-1)d_{p+1} = p^{\Oh(p)}$ many recursive calls, where $d_{p+1}$ denotes the $(p+1)$ th Bell's number: number of  possible partitions of a set of $(p+1)$ elements. First we take union of all the solution sets corresponding to every recursive calls, specifically, we compute 

    \begin{equation}
        \cF^1(T, p, k) \coloneqq \bigcup_{v \in S} \cF^1_v \cup  \bigcup_{(C_t, \cP, p_1) \in {\cal G}_t} \cF^1(C_t, \cP, p_1)  \cup \bigcup_{(C_s, \cP, p_1) \in {\cal G}_s} \cF^1(C_t, \cP, p_1). \label{eqn:repsetcomputation1}
    \end{equation}
    Then we compute 
     \begin{equation}
         \cF'(T, p, k) \repset{q} \cF^1(T, p, k) \label{eqn:repsetcomputation2}
     \end{equation}
    using \Cref{prop:repset} and return the set $\cF'(T, p, k)$ as the output for the instance $\cJ = (G,\cM, T, p, q)$.  
	
	%$$\cF^1(T, p, k) \coloneqq \lr{\bigcup_{v \in S} \cF^1(v) } \cup \lr{\bigcup_{(C_t, \cP, p_1) \in {\cal G} } \cF^1(C_t, \cP, p_1) }.$$ 
	
	
	% We will return $\cF'(T, p, k) \repset{q} \cF^1(T, p, k)$.  
	
	%\todo{Define ${\cal G}$ as the collection of all tuples $(C_t, \cP, p_1)$ of guesses.
	
\end{description}
This finishes the description of \mwcut.






\subparagraph{Correctness.}

	\begin{lemma}[Safeness of \mwcut]
		Our branching algorithm returns the set  $\cF'(T, p, G) \repset{q} \cF(T, p, G)$ of size $2^{p+q}$.  
	\end{lemma}
	\begin{proof}
		Recall that $\cF(T, p, G)$ is the set of all minimal independent multiway cuts for $T$ of size $p$ in $G$. First, we consider base case, then the correctness follows from \Cref{cl:basecase}.         Now, suppose that neither of the base cases is applicable. If the graph $G$ is disconnected, then again the correctness of the algorithm follows directly from \Cref{cl:disconnected}.        Hence, finally let us consider the case when $G$ is connected, $p \ge 2$, and $|T| \ge 3$.  
        First, by \Cref{lem:strong}, we either correctly conclude that $\cJ = (G, \cM, T, p, q)$ is a \no-instance, or we find a strong separator $S$ and a pair of components $C_s, C_t$ in time $2^p \cdot n^{\Oh(1)}$, such that for any minimal solution $O \in \cF(G, T, p)$ of size $p$, either (i) $S \cap O = \emptyset$, (ii) $1 \le |C_s \cap O| \le p-1$, or (iii) $1 \le |C_t \cap O| \le p-1$. Further, any $O$ satisfying (ii) (resp.~(iii)) must be compatible  with some guess $(C_t, \cP, p_1) \in {\cal G}_t$ (resp.~$(C_s, \cP, p_1) \in {\cal G}_s$) (by \cref{claim:compatible}. 
        This implies that, 
        \begin{align}
            \cF(T, p, G) = \bigcup_{v \in S} \cF(T, p, v, G) \ \cup  &\bigcup_{(C_t, \cP, p_1) \in {\cal G}_t} \cF(T, p, G, C_t, \cP, p_1)  \nonumber
            \\&\cup \bigcup_{(C_s, \cP, p_1) \in {\cal G}_s} \cF(T, p, G, C_s, \cP, p_1).
        \end{align}
        Then, by \Cref{cl:s-branchingrepset,cl:divide}, it follows that $\cF^1(T, p, G) \repset{q} \cF(T, p, G)$, where the former is defined in \eqref{eqn:repsetcomputation1}. Then, since $\cF'(T, p, G) \repset{q} \cF^1(T, p, G)$ as computed in \eqref{eqn:repsetcomputation2}, by \Cref{obs:repsetprops}, it follows that $\cF'(T, p, G) \repset{q} \cF(T, p, G)$. Finally, by \Cref{prop:repset}, it follows that $|\cF'(T, p, G)| \le 2^{p+q}$. 
        
        %for any $O \in \cF(G, T, p)$, either $O \in \cF(T, p, v, G)$, or $O$ is compatible with some guess $(C_t, \cP, p_1) \in {\cal G}_t$ or with $(C_s, \cP, p_1) \in {\cal G}_s$. As a corollary, if $\cF(G, T, p) = \emptyset$, then for all $v \in S, \cF(T, p, v, G) = \emptyset$, for all guesses $(C_t, \cP, p_1) \in {\cal G}_t$, $\cF(T, p, G, C_t, \cP, p_1) = \emptyset$, and for all guesses $(C_s, \cP, p_1) \in {\cal G}_t$, $\cF(T, p, G, C_t, \cP, p_1) = \emptyset$. Then, by \Cref{cl:s-branchingrepset,cl:divide}, it follows that $\cF^1(T, p, k) = \emptyset$, which implies that the output of the algorithm, i.e., $\cF'(T, p, G) \repset{q} \cF^1(T, p, G)$ satisfies that $\cF'(T, p, G) = \emptyset$.  
        \iffalse
        Next, consider that $\cF(T, p, G) \neq \emptyset$, and consider any $O \in \cF(T, p, G)$. Further, let $Y \subseteq U(\cM)$ of si
        %We show that our algorithm returns a set $ \cF'(T, p, G) \repset{q} \cF(T, p, G)$. Since $\cF'(T, p, G) \repset{q} \cF^1(T, p, G)$, by \Cref{obs:repsetprops}, it suffices to show that $\cF^1(T, p, G) \repset{q} \cF(T, p, G)$.  
		
		Let $Y \subseteq V(G)$ be a set of size $q$ such that there is a set $O  \in \cF(T, p, G)$  such that $O $ fits $Y$.   We have to show that there is a $\hat{X}  \in \cF^1(T, p, G)$ such that$\hat{X}$ fits $Y$ and that is also minimal multiway cut of size $p$ in $G$. 
		 Now we have several cases depending on the set $Y$ and $S$.
		
		\begin{description}[leftmargin=7pt]
					
			\item[Case 1: $X \cap S \neq \emptyset$. \label{case:intersect}] Let $v$ be a vertex in $X \cap S$. Then consider $\cF'_v$, which is a $q$-representative ser of all independent minimal multiway cuts of $T$ that contains $v$ (by \cref{claim:}). As by our construction of $ \cF^1(T, p, G) $, the set $\cF'_v$ is contained in $\cF^1(T, p, G) $ we are done.
			
			\item[Case 2: $X \cap S = \emptyset$. \label{case:nonintersect}] As $S$ is strong separator, so there must exist a terminal component in $G-S$ which has a non-empty intersection with at most $p-1$ vertices of $O$. Consider such terminal component $C_t$ with terminal vertex $t$. Let $|O \cap V(C_t)| =p_1$ and $\cP$ be the partition of vertices in $\reach{t} \cup \{t\}$ in the graph $G_1= G[V(C_t) \cup \reach(t)]$ such that for each pair of vertices $u, v$ in $\reach{t} \cup \{t\}$ belongs to different part if they are not connected in the graph $G_1 \setminus O$. Now  consider $\cF'(C_t, \cP, p_1)$, which is a $q$-representaive ser of all independent minimal multiway cuts of $T$ that are compatible with the guess $(C_t, \cP, p_1)$.  As by our construction of $ \cF^1(T, p, G) $, the set $\cF'(C_t, \cP, p_1)$ is contained in $\cF^1(T, p, G) $ we are done.
			
			
		\end{description}
        \fi
		\end{proof}
	
	\subparagraph{Time analysis.}
	
	Note that in each of the recursive calls to our branching steps, the parameter $p$ decreases by at least $1$. The number of partition of the vertices in $S$ is bounded by $p^p$. So the degree at each node of the branching tree is bounded by $p^{\cO(p)}$. In the base case where $|T|=2$ or $p=1$ we found the corresponding solution in {\color{red} stcut time}. The number of nodes in the tree is bounded by $p^{\cO(p)}$. Now we calculate the running to find a solution to each node assuming that we have all the solution to its child node. For this, we have to take union of at most $(p+ 2(p-1)(p+1)^{p+1})^p$ many sets where the size of each set is at most $\binom{p+q}{p}$. This union takes $\binom{p+q}{p} \cdot (p+ 2(p-1)(p+1)^{p+1})^p$ time. Then finding the $q$-representative set will take time $\mathcal{O}(\binom{p+q}{p}tp^\omega+t\binom{p+q}{q}^{\omega-1})+\|A\|^{\mathcal{O}(1)}$. 
	
	
	\medskip 
	
	Hence, we have the following theorem.
	
	\begin{restatable}{theorem}{multiwaycuttheorem} \label{thm:multiwaycuttheorem}
	There exists a deterministic algorithm for {\sc Generalized} \probmwcut that runs in time $2^{p+q} \cdot n^{\Oh(1)}$ \todo{time should be way higher than this}, and outputs $\cF'(T, p,G) \repset{q} \cF(T, p, G)$ such that $|\cF'(T, p,G)| = 2^{p+q}$. Here $\cF(T, p, G)$ denotes the set of all $p$ size multiway cut for $T$ in $G$. 
	%Given an undirected  graph $G$, a pair of vertices $s,t$, a matroid $\M= (V, \cI)$ of rank $r$, an integer $k \leq r$, in $f(k,r) \cdot n^{\cO(1)}$, 
	
	%time we either say there is no vertex \stc of size at most $k$, or, a $(r-k)$-representative family $ \mathcal{F}' \subseteq^{r-k}_{\text{rep}} \mathcal{F}$  of size at most $ g(k,r) $ of all independent $s$-$t$ cuts $\mathcal{F}$ of size $k$ in $G$.
\end{restatable}

{\color{red} To do
\begin{itemize}
     \item time analysis (after st cut)
       \item Final theorem statement modify
    \item two figures

 
    \item fix $p \rightarrow k, q \rightarrow r-k$
    
\end{itemize}}










\newpage 



















==> note.tex <==


Q1) Why is a minimum s-t cut not sufficient? Why do we require flow?

Answer: 
Let the value of k be 20. However, the minimum cut size is 10. It is possible that there is no independent cut set of size 10. The size of the smallest independent cut set, denoted as S, is 15. We can consider S as minimal because any subset of the independent set is also independent. Additionally, we do not have a method to solve for the minimal cut. Therefore, we utilize flow in order to transform the graph such that the size of the minimum cut set becomes 15, with S becoming the minimum cut set in the new graph. This allows us to solve for the minimum cut effectively.

Q2) Why size of the returned family is $4^k$ for directed vertex s-t cut?

Answer: 
All paths have $t$ as last vertex and no choice for coloring of $t$. for the $k$ vertices in the second last layer, we can only color $b$ or $t$, overall $2^k$ choices for $y$. As there are $2^k$ many coloring that colors the vertex $t$ tan and each entry store $2^k$ many sets, so size of the family is $4^k$. 


Q3) Satya

    \item $ \Pi_1 \rightarrow \Pi_2 :$ If we can solve $ \Pi_2 $ then we are done for $ \Pi_1 $.
     
    \item  Undirected vertex cut $ \rightarrow $ Directed vertex cut: Replace every undirected edge with forward and backward arcs. 
    	
    \item Directed vertex cut $ \rightarrow $ Directed edge cut: Split each vertex $ v $ into $ v_{\text{in}} ,  v_{\text{out}} $ and add an arc $ ( v_{\text{in}} ,  v_{\text out}) $. Furthermore, for each original arc $ (u,v) $, add $ k+1 $ parallel arcs $ (u_{\text{out}},  v_{\text{in}}) $. 

    \item Directed vertex cut $ \rightarrow $ Directed edge cut: Split each vertex $ v $ into $ v_{\text{in}} ,  v_{\text{out}} $ and add an arc $ ( v_{\text{in}} ,  v_{\text out}) $. Furthermore, for each original arc $ (u,v) $, add arc $ (u_{\text{out}},  v_{\text{in}}) $. Proof: Because in reverse direction if some $(u_{\text{out}}, v_{\text{in}})$ is chosen in edge cut solution, then we can replace it with $(v_{\text{in}}, v_{\text{out}})$ or $(u_{\text{in}}, u_{\text{out}})$ and kill the same set of paths.
      
        	
    \item Directed edge cut $ \rightarrow $ Directed vertex cut: for each original vertex $ u $, make $ k+1 $ copies $ u_1, u_2, \ldots, u_{k+1}$.  For each original arc $ (u,v) $, add a vertex $ e_{uv} $, and add arcs $ (u_i, e_{uv}) $ and $ (e_{uv}, v_i) $  for $i = 1, \ldots , k+1$.


     \item Directed edge cut $ \rightarrow $ Directed vertex cut: for each  original arc $ (u,v) $, add a vertex $ e_{uv} $, and add arcs $ (u, e_{uv}) $ and $ (e_{uv}, v) $.

     \item Undirected edge cut $\rightarrow$ Undirected vertex cut: (Similar reduction as we used for Directed edge cut $ \rightarrow $ Directed vertex cut)  -- for each original vertex $ u $, make $ k+1 $ copies $ u_1, u_2, \ldots, u_{k+1}$.  For each original edge $e = uv$, add a vertex $ e_{uv} $, and add edges $ u_ie_{uv}) $ and $ e_{uv}v_i$  for $i = 1, \ldots , k+1$.

     % Reducing Edge Connectivity to Vertex Connectivity       	    	
    	
    \item Directed vertex cut $ \rightarrow $  Undirected vertex cut

    \item Directed edge cut $ \rightarrow $  Undirected edge cut

    \item Undirected vertex cut $ \rightarrow $  Undirected edge cut



(Q4) Difference between oracle and rep set.

Oracle is weaker than representation Power of oracle: We can ask one query then in unit/poly time he will answer it correctly. But in reresentation we can work, .e.g, we can find rep set of certain size which we can not do in oracle. Another thing is that in oracle we need to make so many query to return our solution as if we do less then adversary can change the oracle that compatible with previous answer but answer becomes wrong. One such example is: given a binary string of size $n$, we need to query $n$ call to produce answer. If we do less than that then adversary can change the binary string and make our answer wrong.



(Q4) Why minimal cut = k not work?

Let size of minimum non-ind cut = 30, 
size of minimum ind cut = 50

Suppose F(s,t,60)= set of all minimal independent cuts of size 60.
Now fix a Z: minimal cut of size 60. We know that there is A such that, in G+A, Z becomes the minimum cut.
Let there be some Z' of size 60 in G such that in G that is not minimal but in G+A the set Z' is minimum. Now there is some Z'' \subset Z' which is minimal in G.

Now, if we compute the rep set for F(s,t,60), that is not enough. Because we are not considering Z' there. But there may be some Y that fits both Z and Z'.  As we are not considering Z', we might miss the rep set of all solutions. Notice that if Y fits Z' it will also fit Z''.

one option: F(s,t,60)= set of all minimal independent cuts of size at most 60. 

(Q5) Why minimum independent cut will work?

F(s,t,60)= set of all minimum independent set of size 60. Where 60= size of a minimum independent cut. 

Now min cut size may be 40.

Now Any S in F (s,t,60) may not be minimum cut but must be minimal cut. that's why we add A such that S become minimum cut in G+A.

Now, if we compute the rep set for F(s,t,60), it is enough. Because there is no Z of size 80 (basically more than 60) in G which will become minimum in the new graph. 

(Q5) There are many way to handle branching case for terminal components, but we have to make sure that solution does not take the merge vertices:
  [1] -- Change the instance to (G, M, T, p, q, L) where V(G)-T-L \subseteq U(M)
  [2] -- delete the merge vertex: make clique to their neighbour now any minimal solution will not take the new vertex, also no new path is created
  [3] -- for each merge vertex replace with (k+1)-similar vertices 
  
